Common Subcontracting and Airline Prices

In the US airline industry, independent regional airlines fly passengers on behalf of several national airlines across different markets, giving rise to $\textit{common subcontracting}$. On the one hand, we find that subcontracting is associated with lower prices, consistent with the notion that regional airlines tend to fly passengers at lower costs than major airlines. On the other hand, we find that $\textit{common}$ subcontracting is associated with higher prices. These two countervailing effects suggest that the growth of regional airlines can have anticompetitive implications for the industry.

==> tables_tex/weather_firststage_averages.tex <==
\begin{tabular}{lcc} \toprule
{Variables} &  Common Subcontracting (CSC) & Regional Share\\
\midrule
IV Mean Precipitation (tenths of mm) & 0.0000127* & 0.0008501*** \\
 &  (0.00000727)  & (0.0000284) \\
IV Mean Snowfall (mm)   & 0.00114*** & 0.0392***    \\
 &  (0.000278) & (0.00135) \\
IV Mean Snow Depth (mm) & 0.000902*** & -0.000378    \\
 &  (0.000152) & (0.000507) \\
IV Mean Minimum Temp (tenths of degrees celsius) & 0.000157*** & 0.000059** \\
 & (0.00000516) & (0.0000267) \\
 Regional Network IV & 0.000347*** & \\
 & (0.00000358) & \\
\midrule
\emph{F-stats (instruments):}& 1,271.85 & 661.49  \\
\midrule
Observations & 1,000,180 & 1,000,180 \\
Number of markets & 21,390 & 21,390\\
R$^2$ & 0.51  & 0.29 \\
\bottomrule
\end{tabular}



==> tables_tex/weather_firststage_extremes.tex <==
\begin{tabular}{lcc} \toprule
{Variables} &  Common Subcontracting (CSC) & Regional Share\\
\midrule
IV Worst Precipitation (tenths of mm) & 0.00000345 & 0.000286*** \\
 &  (0.00000388)  & (0.0000154) \\
IV Worst Snowfall (mm)   & 0.000686*** & 0.0118***    \\
 &  (0.000105) & (0.000457) \\
IV Worst Snow Depth (mm) & 0.000332*** & -0.000405***    \\
 &  (0.0000585) & (0.000195) \\
IV Worst Minimum Temp (tenths of degrees celsius) & 0.0000832*** & 0.000208***\\
 & (0.00000513) & (0.0000218) \\
 Regional Network IV & 0.000344*** & \\
 & (0.00000359) & \\
\midrule
\emph{F-stats (instruments):}& 1,240.34 & 650.00  \\
\midrule
Observations & 1,000,180 & 1,000,180 \\
Number of markets & 21,390 & 21,390\\
R$^2$ & 0.51  & 0.29 \\
\bottomrule
\end{tabular}



==> tables_tex/weather_iv_robust.tex <==
\begin{tabular}{lc} \toprule
{Variables} &  (1) \\
\midrule
Common Subcontracting (CSC)  & 0.0789*** \\
 & [.00735]  \\
{Regional Share}   & -0.216***    \\
 & [0.0213]  \\
Multimarket Contact (MMC) & 0.0235***    \\
 &  [0.000764] \\
\midrule
{\bf First-Stage Results} &\\
 &  \\
\emph{Residuals:} CSC  & -0.0996***  \\
 &  [0.00816]\\
{Regional Share}  & 0.248***  \\
&  [0.0214]\\
MMC & -0.0158***  \\
 &  [0.000949]\\
\emph{F-stats (instruments):}  CSC& 1,271.85   \\
 Regional Share &  661.49 \\
MMC &    5,350.11 \\
\midrule
Observations & 1,000,180  \\
Number of markets & 21,390 \\
R$^2$ & 0.094  \\
\bottomrule
\end{tabular}


